The Einstein Probe transient EP240414a: Linking Fast X-ray Transients, Gamma-ray Bursts and Luminous Fast Blue Optical Transients

Detections of fast X-ray transients (FXTs) have been accrued over the last few decades. However, their origin has remained mysterious. There is now rapid progress thanks to timely discoveries and localisations with the Einstein Probe mission. Early results indicate that FXTs may frequently, but not always, be associated with gamma-ray bursts (GRBs). Here, we report on the multi-wavelength counterpart of FXT EP240414a, which has no reported gamma-ray counterpart. The transient is located 25.7~kpc in projection from a massive galaxy at $z=0.40$. We perform comprehensive photometric and spectroscopic follow-up. The optical light curve shows at least three distinct emission episodes with timescales of $\sim 1, 4$ and 15 days and peak absolute magnitudes of $M_R \sim -20$, $-21$, and $-19.5$, respectively. The optical spectrum at early times is extremely blue, inconsistent with afterglow emission. It may arise from the interaction of both jet and supernova shock waves with the stellar envelope and a dense circumstellar medium, as has been suggested for some Fast Blue Optical Transients (LFBOTs). At late times, the spectrum evolves to a broad-lined~Type~Ic supernova, similar to those seen in collapsar long-GRBs. This implies that the progenitor of EP240414a is a massive star creating a jet-forming supernova inside a dense envelope, resulting in an X-ray outburst with a luminosity of $\sim 10^{48}$ erg s$^{-1}$, and the complex observed optical/IR light curves. If correct, this argues for a causal link between the progenitors of long-GRBs, FXTs and LFBOTs.

==> authors.tex <==
% author list
\author[1]{\fnm{Joyce N. D.} \sur{van Dalen}}
%\email{joyce.vandalen@ru.nl}

\affil[1]{\orgdiv{Department of Astrophysics/IMAPP}, \orgname{Radboud University Nijmegen}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\author[1]{\fnm{Peter G.} \sur{Jonker}}
%\email{p.jonker@astro.ru.nl}

%\affil[1]{\orgdiv{Department of Astrophysics/IMAPP}, \orgname{Radboud University Nijmegen}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\author[1,2]{\fnm{Andrew J.} \sur{Levan}}\email{a.levan@astro.ru.nl}

%\affil[1]{\orgdiv{Department of Astrophysics/IMAPP}, \orgname{Radboud University Nijmegen}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\affil[2]{\orgdiv{Department of Physics}, \orgname{University of Warwick}, \orgaddress{\street{Coventry, CV4 7AL}, \country{UK}}}

\author[4,5,1]{\fnm{Daniele Bj\o{}rn} \sur{Malesani}}%\email{daniele.malesani@nbi.ku.dk}
\affil[4]{\orgdiv{Cosmic Dawn Center (DAWN)}, \orgaddress{\country{Denmark}}}
\affil[5]{\orgdiv{Niels Bohr Institute}, \orgname{University of Copenhagen}, \orgaddress{\street{Jagtvej 128}, \city{Copenhagen}, \postcode{2200}, \country{Denmark}}}
%\affil[1]{\orgdiv{Department of Astrophysics/IMAPP}, \orgname{Radboud University Nijmegen}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\author[1]{\fnm{Jonathan} \sur{Quirola-V\'asquez}}
%\email{jaquirola@uc.cl}
%\affil[1]{\orgdiv{Department of Astrophysics/IMAPP}, \orgname{Radboud University Nijmegen}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\author[9,10]{\fnm{Daniel} \sur{Mata S\'anchez}}  
\affil[9]{\orgdiv{Instituto de Astrof\'{i}sica de Canarias}, \orgname{IAC}, \orgaddress{\street{E-38205}, \city{La Laguna, S/C de Tenerife}, \country{Spain}}}
\affil[10]{\orgdiv{Departamento de Astrof\'isica, Univ. de La Laguna},   \orgaddress{\street{E-38206}, \city{La Laguna, Tenerife},     \country{Spain}}}

\author[7,5]{\fnm{Luca} \sur{Izzo}}
%\email{luca.izzo@inaf.it}
\affil[7]{\orgdiv{Osservatorio Astronomico di Capodimonte}, \orgname{INAF}, \orgaddress{\street{Salita Moiariello 16}, \city{Napoli}, \postcode{80131},   \country{Italy}}}
%\affil[2]{\orgdiv{Niels Bohr Institute, University of Copenhagen}, \orgname{DARK}, \orgaddress{\street{Jagtvej 128}, \city{Copenhagen}, \postcode{2200},   \country{Denmark}}}

\author[17,18]{\fnm{Antonio} \sur{de Ugarte Postigo}}%\email{deugarte@oca.eu}

\affil[17]{\orgdiv{Universit\'{e} de la C\^ote d'Azur, Observatoire de la C\^ote d'Azur, CNRS, Artemis},   \orgaddress{  \city{Nice}, \postcode{F-06304},   \country{France}}}
\affil[18]{\orgdiv{Aix Marseille Univ, CNRS, LAM}, \orgaddress{\city{Marseille},     \country{France}}}

\author[9,10]{\fnm{Manuel} \sur{A. P. Torres}}%\email{mapt@iac.es}
%\affil[1]{\orgdiv{Instituto de Astrof\'{i}sica de Canarias },\orgname{iac}, \orgaddress{\street{E-38205},\city{La Laguna, S/C de Tenerife}, \country{Spain}}}
%\affil[2]{\orgdiv{Departamento de Astrof\'isica, Univ. de La Laguna, },   \orgaddress{\street{E-38206}, \city{La Laguna, Tenerife},     \country{Spain}}}

\author[1]{\fnm{Maria E.} \sur{Ravasio}}%\email{mariaedvige.ravasio@ru.nl}

%\affil[1]{\orgdiv{Department of Astrophysics/IMAPP}, \orgname{Radboud University Nijmegen}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\author[49,50]{\fnm{Nikhil} \sur{Sarin}}%\email{nikhil.sarin@su.se}
\affil[49]{\orgdiv{The Oskar Klein Centre, Department of Physics}, \orgname{Stockholm University}, \orgaddress{\street{AlbaNova}, \city{Stockholm}, \postcode{SE-106 91}, \state{Stockholm}, \country{Sweden}}}
\affil[50]{\orgdiv{Nordita}, \orgname{Stockholm University and KTH Royal Institute of Technology}, \orgaddress{\street{Hannes Alfvéns väg 12}, \city{Stockholm}, \postcode{SE-106 91}, \state{Stockholm}, \country{Sweden}}}

\author[32]{\fnm{Stuart P.} \sur{Littlefair}}%\email{s.littlefair@sheffield.ac.uk}

%\affil[32]{\orgdiv{Department of Physics and Astronomy}, \orgname{University of Sheffield}, \orgaddress{  \city{Sheffield}, \postcode{S3 7RH},   \country{United Kingdom}}}

\author[28,1]{\fnm{Ashley} \sur{Chrimes}}
%\email{ashley.chrimes@esa.int}

\affil[28]{\orgdiv{European Space Agency (ESA)}, \orgname{European Space Research and Technology Centre (ESTEC)}, \orgaddress{\street{Keplerlaan 1}, \city{Noordwijk}, \postcode{2201~AZ},   \country{The Netherlands}}}
%\affil[2]{\orgdiv{Department of Astrophysics/IMAPP, Radboud University Nijmegen, }, \orgname{IMAPP}, \orgaddress{\street{P.O.~Box 9010}, \city{Nijmegen}, \postcode{6500~GL},   \country{The Netherlands}}}

\author[24,25,26]{\fnm{Franz E.} \sur{Bauer}}
%\email{fbauer@uc.cl}

\affil[24]{\orgdiv{Instituto de Astrof{\'{\i}}sica, Facultad de F{\'{i}}sica and Centro de Astroingenier{\'{\i}}a, Facultad de F{\'{i}}sica, Pontificia Universidad Cat{\'{o}}lica de Chile}, \orgname{UC}, \orgaddress{\street{Campus San Joaquín, Av. Vicuña Mackenna 4860, Macul}, \city{Santiago}, \postcode{7820436}, \state{RM}, \country{Chile}}}
\affil[25]{\orgdiv{Millennium Institute of Astrophysic}, \orgname{MAS}, \orgaddress{\street{Nuncio Monse{\~{n}}or S{\'{o}}tero Sanz 100, Of 104, Providencia}, \city{Santiago}, \postcode{7500011}, \state{RM}, \country{Chile}}}
\affil[26]{\orgdiv{Space Science Institute}, \orgname{SSI}, \orgaddress{\street{4750 Walnut Street, Suite 205}, \city{Boulder}, \postcode{80301}, \state{CO}, \country{USA}}}

\author[27]{\fnm{Francesco} \sur{Carotenuto}}%\email{francesco.carotenuto@physics.ox.ac.uk}

\affil[27]{\orgdiv{Astrophysics, Department of Physics}, \orgname{University of Oxford}, \orgaddress{\street{Keble Road}, \city{Oxford}, \postcode{OX1 3RH},   \country{United Kingdom}}}

% Morgan Fraser

% list of interested from stargate
\author[46]{\fnm{Giovanna} \sur{Pugliese}}%\email{g.pugliese@uva.nl}

\affil[46]{\orgdiv{Anton Pannekoek Institute of Astronomy}, \orgname{University of Amsterdam}, \orgaddress{\street{Science Park 904}, \city{Amsterdam}, \postcode{1098 XH},   \country{The Netherlands}}}

\author[37]{\fnm{Pall} \sur{Jakobsson}}%\email{pja@hi.is}

\affil[37]{\orgdiv{Centre for Astrophysics and Cosmology}, \orgname{University of Iceland}, \orgaddress{\street{Dunhagi}, \city{Reykjav\'ik}, \postcode{107},   \country{Iceland}}}

\author[16]{\fnm{Antonio} \sur{Martin-Carrillo}}
%\email{antonio.martin-carrillo@ucd.ie}

\affil[16]{\orgdiv{School of Physics and Centre for Space Research}, \orgname{University College Dublin}, \orgaddress{\street{Belfield}, \city{Dublin 4},     \country{Ireland}}}

\author[31]{\fnm{Massimiliano} \sur{De Pasquale}}%\email{masdepasquale@unime.it}

\affil[31]{\orgdiv{MIFT Department}, \orgname{University of Messina}, \orgaddress{\street{Via F. S. D'Alcontres 31}, \city{Messina}, \postcode{98166},   \country{Italy}}}

\author[43]{\fnm{Tayyaba} \sur{Zafar}}%\email{tayyaba.zafar@mq.edu.au}

%\affil[43]{\orgdiv{School of Mathematical and Physical Sciences}, \orgname{Macquarie University}, \orgaddress{    \postcode{2109}, \state{NSW}, \country{Australia}}}

\author[6]{\fnm{Paul} \sur{O'Brien}}%\email{pto2@leicester.ac.uk}

%\affil[1]{\orgdiv{School of Physics and Astronomy}, \orgname{University of Leicester}, \orgaddress{\street{University Road}, \city{Leicester}, \postcode{LE1 7RH},   \country{United Kingdom}}}

\author[22]{\fnm{Dong} \sur{Xu}}
%\email{dxu@nao.cas.cn}

\affil[22]{\orgdiv{Key Laboratory of Space Astronomy and Technology, National Astronomical Observatories}, \orgname{Chinese Academy of Sciences}, \orgaddress{\street{20A Datun Road}, \city{Beijing}, \postcode{100101},   \country{China}}}

%Alexander van der Horst
%Jesper Sollerman

